Modeling and Analysis of Utilizing Cryptocurrency Mining for Demand Flexibility in Electric Energy Systems: A Synthetic Texas Grid Case Study

The electricity sector is facing the dual challenge of supporting increasing level of demand electrification while substantially reducing its carbon footprint. Among electricity demands, the energy consumption of cryptocurrency mining data centers has witnessed significant growth worldwide. If well-coordinated, these data centers could be tailor-designed to aggressively absorb the increasing uncertainties of energy supply and, in turn, provide valuable grid-level services in the electricity market. In this paper, we study the impact of integrating new cryptocurrency mining loads into Texas power grid and the potential profit of utilizing demand flexibility from cryptocurrency mining facilities in the electricity market. We investigate different demand response programs available for data centers and quantify the annual profit of cryptocurrency mining units participating in these programs. We perform our simulations using a synthetic 2000 bus ERCOT grid model, along with added cryptocurrency mining loads on top of the real-world demand profiles in Texas. Our preliminary results show that depending on the size and location of these new loads, we observe different impacts on the ERCOT electricity market, where they could increase the electricity prices and incur more fluctuations in a highly non-uniform manner.

==> response_letter.tex <==
\section{Reviews}
Dear Editor in Chief,

We are submitting the revised version of our manuscript titled  ``Modeling and Analysis of Utilizing Cryptocurrency Mining for Demand Flexibility in Electric Energy
Systems: A Synthetic Texas Grid Case Study''. 
We have also given a detailed response to all the questions and comments made by the reviewers and the editor. 

We would like to thank the Editor in Chief and the reviewers for their constructive comments on our manuscript.  We believe that we have addressed all the issues and concerns raised in the reviews.


Sincerely,

\begin{raggedright}
Ali Menati, \\
Kiyeob Lee, \\
Le Xie. \\
\end{raggedright}



\section*{Response to Editor:}
\begin{enumerate}
\item \reviewer{While this paper has some technical merits, the authors should improve the presentation quality of this paper by including most recent works in the literature review and discussing the uncertainties in the problem formulation.}
%{The authors would like to thank the editor and reviewers for the time and effort of going through this manuscript. In this revised manuscript, the comments and issues raised by the reviewers have been carefully addressed. In order to improve the overall readability of the paper, further explanations/clarifications have been made and the new/modified parts of the manuscript are marked in \bluetext{blue}. }
\textcolor{red}{Response:}
The authors would like to thank the editor in chief
for the valuable comments and suggestions. A more comprehensive literature review has been added to the revised manuscript. We introduce previous works on data center operation management and demand response as well as cryptocurrency mining impact on the grid. We have added more clarification of the problem formulation and the uncertainty involved in the decision-making process. These changes can be found in section 4 of the revised manuscript. 

We performed new simulations with uncertain electricity prices to clarify the impact of uncertainty on cryptominers demand response profit. To this end, ERCOT electricity price records from 2019 to 2021 are obtained, and their distribution is used to add random noise on top of the hourly LMPs obtained by solving SCED. By repeating our simulations 1000 times, the mean, upper bound, and lower bound of the demand response profit are calculated. The updated results are shown in Figure 8 of section 6, where the simulation setting is also updated.


\end{enumerate}
\section*{Response to Reviewer 1}

\begin{enumerate}
    \item \reviewer{As Sections 2 and 3 are not the contributions of the authors, it is suggested to be shortened; in this version, they are too long.}

    \textcolor{red}{Response:} The authors would like to thank the reviewer for constructive comments and great suggestions. Per your suggestion we have shortened section 2 and 3, by removing some contents and summarizing other. These changes can be seen in the revised manuscript. 
    
       \item \reviewer{Equation (1) models the optimization problem of the paper. It is understandable that the authors tried to present a very simple model to show the impact of mining load on the Grid's flexibility, but I believe that oversimplification can mislead the results. For example, $p_b$ and $p_e$, which indicate the predicted revenue from selling the mined cryptocurrency and the cost of electricity per unit, are better to be modeled as time-dependent non-constant parameters with sources of uncertainty. Indeed, considering the uncertainties on electricity and cryptocurrency prices, this is highly recommended.}
       
       \textcolor{red}{Response:} Thanks for raising this valuable question. The authors are currently investigating more complicated models capable of capturing a realistic uncertainty setting.  Uncertainties in electricity and cryptocurrency prices will definitely change the optimization (decision) variables, i.e., how much MW to participate in each demand response program at any given time. In our current formulation we consider both electricity price $\hat{p_e}(t)$ and Bitcoin price $\hat{p_b}(t)$ as uncertain values that change over time. Hence our mining profit $\hat{r}(t)= \hat{p_b}(t)-\hat{p_e}(t)$ is also changing and comes with uncertainty. While our problem formulation considers these uncertainties, we solve a simpler version of the problem, where we assume an expected value of the future information is obtained through prediction and historical records. To clarify our setting and the uncertainties involved in the decision-making process, a more detailed discussion of the problem formulation has been added to section 4 of the revised manuscript.
       
       Per your suggestion, we also designed a new simulation setting to capture the impact of uncertain electricity prices on cryptominers demand response profit. We obtained ERCOT electricity price records for the year 2019 to 2021 and used their distribution to add random noise on top of the hourly LMPs obtained by solving SCED. Repeating the simulations 1000 times gives us the mean, upper bound, and lower bound of the demand response profit. As shown in Figure 8, the difference between the upper bound and lower bound clearly captures the impact of the electricity price uncertainty on cryptominers' demand response profit. The updated results and our clarifications can be found in section 6-D of the revised manuscript.
\end{enumerate}


\section*{Response to Reviewer 2}
\begin{enumerate}
    \item \reviewer{The literature review is not sufficient. It is recommended to provide a detail literature review by analyzing papers that study energy management in datacenters which participate to demand response programs.}

    \textcolor{red}{Response:} The authors would like to thank the reviewer for
constructive comments. We agree that there is a rich literature that studies demand response in data centers \cite{liu2013data,wierman2014opportunities,Tran16, Bahrami19}. One major difference between conventional data centers and mining facilities is that data centers always have a sizable portion of inflexible loads to provide services, but mining facilities can be completely turned-off when needed. This was indeed observed in July 2022 when heat waves hit Texas for an extended time period and mining facilities turned off for the whole time due to high electricity prices. On the other hand, data centers had to still operate and provide services. However, the authors agree that it is fair to include previous works on the energy management in data centers. A more comprehensive literature review of data centers’ workload management and scheduling \cite{Rao12, liu2013data, Ghamkhari13, Chen16}, is included in the current version, along with a review of utility companies’ optimal pricing mechanisms to encourage data centers participation in demand response \cite{Wang16, liu2011greening, Tran16}. We also included some previous works analysing the impact of Bitcoin mining loads on the power gird \cite{Moghimi21, KARMAKAR2021110111}. 

    \item \reviewer{The simulation results are predictable. It is expected to obtain higher electricity price result and some grid congestion when high amount of load is integrated into the grid. The same result can be anticipated for the integration of electrical vehicles. What do the results indicate/show for the load increase with cryptocurrency mining different than electrical vehicles for instance?}

    \textcolor{red}{Response:} Thanks for raising this valuable question. While there are similarities between mining loads and EV loads, there are also fundamental differences between these two in terms of integration and their participation in demand response. We briefly list these differences as follows:
    1- Potential demand response capacity of EVs depeneds on their consumption patterns and duration curve. While EVs available capacity constantly changes over time, Bitcoin mining demand response capacity is almost fixed and instantaneous. 2- EVs are distributed across the system in a non-uniform manner and demand response aggregators need to collect a lot of EVs to have the same capability as a mining facility. On the other hand, Mining loads are centralized with clear control strategies for fast change in their consumption levels depending on the price signals and incentives. 3- EVs connectivity to the grid and their adoption are largely subject to socio-economic and behavioral decisions, which makes their consumption patterns highly uncertain and dependent on exogenous factors. On the other hand, mining loads tend to be stable and their internal preference for mining all the time makes them a reliable source of demand response. All in all, the impact of EVs and mining loads on the electricity market is expected to be different, and some comparative studies are suggested, but that is out of the scope of this paper.
    
    
    \item \reviewer{The impact of the demand flexibility should be analyzed by performing simulations with the same algorithm (for cryptocurrency mining load) with/without participating the demand response program. After then, the impact of the demand response on cryptocurrency mining can be investigated. Currently, this comparison is not available on the results.}

    \textcolor{red}{Response:} The authors would like to thank the suggestion. Although this paper does not explicitly compare different demand response algorithms, our simulation results compare two cases a) existing system without mining loads and b) existing system with different amounts of mining loads. For example, in Fig. 6b the amount of mining load changes between 0 and 840 MW. The authors predict that, when mining facilities participate in a demand response program, the results lie between a) and b) in terms of their impacts. For example, when high LMP is expected and mining facilities reduce their consumption by 100\%, then it results in case a). On the other hand when mining facilities reduce their consumption by 40\%, its impact on the grid lies within the scenarios investigated in our simulations. Hence, the existing system without any mining loads serves as a case study of the mining facility participating in the demand response program with full capacity. Considering your suggestion, we have added a paragraphs clarifying this point at the end of section 6-B of the revised manuscript.


    \item \reviewer{According to results, there is congestion problem and electricity price increase when the huge amount of load is integrated to the grid as expected. In this case, authors suggest what type of novel solution for facilitating the integration of these resources in the demand response market?}
    
    \textcolor{red}{Response:} The authors would like to thank the reviewer for a great question. The authors are currently investigating multiple win-win mechanisms between mining facilities and the system operators. There are multiple angles such as demand response markets, reliability, ancillary services, and carbon reductions that need to be investigated. As presented in the discussion section of the paper, one way to reduce the disruptive impact of these new loads is placing them in locations with more renewables, which reduces electricity prices, carbon footprint, and curtailment in the system. Demand flexibility also plays a pivotal rule, where a few hours of flexibility per day could mitigate the adverse impact of the mining loads on the congestion patters. Another possible strategy is having mining facilities to invest in renewable generation units to cover a certain percentage of their operational capacity. Considering your suggestion, these strategies are all presented in the discussion section of the revised manuscript. 
\end{enumerate}





